Empowering Collaborative Filtering with Principled Adversarial Contrastive Loss

Contrastive Learning (CL) has achieved impressive performance in self-supervised learning tasks, showing superior generalization ability. Inspired by the success, adopting CL into collaborative filtering (CF) is prevailing in semi-supervised top-K recommendations. The basic idea is to routinely conduct heuristic-based data augmentation and apply contrastive losses (e.g., InfoNCE) on the augmented views. Yet, some CF-tailored challenges make this adoption suboptimal, such as the issue of out-of-distribution, the risk of false negatives, and the nature of top-K evaluation. They necessitate the CL-based CF scheme to focus more on mining hard negatives and distinguishing false negatives from the vast unlabeled user-item interactions, for informative contrast signals. Worse still, there is limited understanding of contrastive loss in CF methods, especially w.r.t. its generalization ability. To bridge the gap, we delve into the reasons underpinning the success of contrastive loss in CF, and propose a principled Adversarial InfoNCE loss (AdvInfoNCE), which is a variant of InfoNCE, specially tailored for CF methods. AdvInfoNCE adaptively explores and assigns hardness to each negative instance in an adversarial fashion and further utilizes a fine-grained hardness-aware ranking criterion to empower the recommender's generalization ability. Training CF models with AdvInfoNCE, we validate the effectiveness of AdvInfoNCE on both synthetic and real-world benchmark datasets, thus showing its generalization ability to mitigate out-of-distribution problems. Given the theoretical guarantees and empirical superiority of AdvInfoNCE over most contrastive loss functions, we advocate its adoption as a standard loss in recommender systems, particularly for the out-of-distribution tasks. Codes are available at https://github.com/LehengTHU/AdvInfoNCE.

==> backup/0_abstract.tex <==
\begin{abstract}
Contrastive learning (CL) has achieved impressive performance in self-supervised learning tasks. 
Inspired by this success, CL-based collaborative filtering (CF) has recently emerged for semi-supervised Top-K recommendation \wx{and achieved significant performance gains.
The basic idea is} routinely adopting heuristic-based data augmentation and utilizing contrastive losses like InfoNCE.
However, CF methods face unique challenges due to factors such as Top-K evaluation, Missing-Not-At-Random, and the risk of false negatives.
These challenges necessitate CL-based CF methods to heavily rely on mining hard negatives and distinguishing false negatives for informative training signals.
Furthermore, the understanding of contrastive loss in Top-K evaluation especially its superior robustness remains largely unexplored.

In this paper, we delve into the reasons underpinning the success of contrastive loss in CF and develop an efficient, slightly modified version of InfoNCE loss that adaptively assigns hardness to negative samples.
Grounded in theoretical findings, we propose a principled \textbf{Adv}ersarial \textbf{InfoNCE} loss, termed \textbf{AdvInfoNCE}, ensuring top-tier performance in Top-K recommendation under adversarial hard negative mining conditions, while effectively tackling out-of-distribution problems.
% Specifically, based on theoretical discovery, we propose a principled adversarial contrastive loss, termed \textbf{AdvInfoNCE}, which guarantees Top-K recommendation performance under adversarial hard negative mining and effectively addresses out-of-distribution problems.
% Through extensive experiments on both synthetic and real-world benchmark datasets, we demonstrate the generalization ability of AdvInfoNCE, showcasing its effectiveness in handling out-of-distribution problems. 
Extensive experiments on both synthetic and real-world benchmark datasets underscore the generalization capability of AdvInfoNCE, highlighting its proficiency in managing out-of-distribution problems.
Given the theoretical guarantees and empirical superiority of AdvInfoNCE over existing contrastive loss functions, we advocate its adoption as a standard loss in recommender systems, particularly for out-of-distribution tasks.
Codes are available at \url{https://github.com/}.
\end{abstract}

==> backup/1_introduction.tex <==
\section{Introduction} 
% Contrastive learning (CL) has significantly advanced self-supervised learning tasks \cite{SimCLR, MoCo, Barlow_Twins, SimSiam}, given its notable generalization ability.
% % Contrastive learning (CL) has achieved a significant milestone for its generalization ability over a variety of self-supervised learning tasks \cite{SimCLR, MoCo, Barlow_Twins, SimSiam}.
% By simultaneously maximizing the similarity among positive pairs and pushing apart negative pairs in the feature space \cite{alignment_uniformity}, CL has demonstrated in extracting general features from limited signals.
% % This success has spurred a wave of interest in developing CL-based collaborative filtering (CF) methods for Top-K recommendation tasks \cite{DHCN, KMCLR, S2-MHCN, S3-Rec}, resulting in substantial performance gains.
% The resulting success has ignited interest in developing CL-based collaborative filtering (CF) methods for Top-K recommendation tasks \cite{DHCN, KMCLR, S2-MHCN, S3-Rec, InvCF}, leading to considerable performance improvements.
% The majority of CL-based CF methods follow a standard paradigm, often routinely adopting heuristic-based data augmentation of user-item bipartite graphs \cite{SGL, CLRec, AutoCF}, and blindly utilizing the contrastive losses, such as InfoNCE \cite{InfoNCE}.
% A key implicit assumption underpinning prevailing CL-based CF methods is that all unobserved interactions are considered negative instances \cite{DNS}.

Contrastive Learning (CL) has emerged as a potent tool in self-supervised learning tasks \cite{SimCLR, MoCo, Barlow_Twins, SimSiam}, given its superior generalization ability.
By simultaneously pulling positive pairs close together while pushing apart negative pairs in the feature space \cite{alignment_uniformity}, CL has demonstrated extracting general features from limited signals.
This promising result has propelled research interest in leveraging CL for Collaborative Filtering (CF) in Top-K recommendation tasks, leading to a marked enhancement in performance \cite{DHCN, KMCLR, S2-MHCN, S3-Rec, InvCF}.
Specifically, the prevalent paradigm in CL-based CF methods is to routinely adopt heuristic-based data augmentation for user-item bipartite graphs \cite{SGL, CLRec, AutoCF}, coupled with the indiscriminate application of contrastive losses such as InfoNCE \cite{InfoNCE}. 
A common assumption underlying these methods is considering all unobserved interactions as negative signals \cite{DNS}.

% In spite of the empirical success and notable advancements in CL-based CF methods, 
% we identify and substantiate two key limitations that impede future progress in this direction:
Despite the empirical success of CL-based CF methods, two critical limitations have been observed that potentially impede further advancements in this research direction:
\begin{itemize}[leftmargin=*]
\item \textbf{Lack of a tailored inductive bias for CF.}
% Differ from the effectiveness of instance discrimination in self-supervised learning, CF recommenders face unique challenges such as the positive-unlabeled \cite{Missing-Not-At-Random} and Missing-Not-At-Random problems \cite{DR}. 
% Most interaction data are unobserved, and the lack of interaction does not necessarily signify a negative response. 
% The incorporation of these false negatives would provide erroneous signals for representation learning and seriously degrade the recommendation accuracy \cite{RINCE}. 
% Such prior inductive bias makes the CL-based CF methods heavily rely on mining hard negatives and distinguishing false negatives for providing proper and informative signals \cite{HDCCF}.
% In other words, uniformly treating all unobserved interactions as negatives contradicts real-world scenarios, thus ultimately leading to sub-optimal representation learning.
As a standard approach for semi-supervised Top-K recommendation with implicit feedback, CF methods face unique challenges.
In most cases, the majority of user-item interactions are unobserved and assigned unlabeled, where CF methods directly draw negative instances from.
However, indiscriminately treating these unobserved interactions - more likely to be false negatives - as negative instances is widely acknowledged as insufficient to provide reliable and high-quality contrastive signals \cite{RINCE}, known as the positive-unlabeled issue \cite{Missing-Not-At-Random, DR} in recommender systems.
% This arises in severe noise-injected observations, where the majority of unobserved interactions are false negatives, well-known as the positive-unlabeled issue \cite{Missing-Not-At-Random, DR} in recommender systems. 
% Blindly treating these false negatives as true negatives could generate misleading signals for representation learning, substantially reducing the recommendation accuracy \cite{RINCE}.  
Unfortunately, this inherent inductive bias is rarely considered in current CL-based CF methods, resulting in suboptimal recommendation quality and generalization ability \cite{HDCCF}. 
% heavily rely on false negative identifying and high-quality hard negative mining \cite{HDCCF}.
%, implying that treating all unobserved interactions as negatives uniformly is not reflective of real-world scenarios and may result in sub-optimal representation learning.

% \item \textbf{Limited theoretical understanding for generalization ability in Top-K evaluation.}
% It has been shown in many works that, unlike the important role of data augmentation in computer vision \cite{epsilon-delta, ConnectNotCollapse}, the CL-based CF model is not sensitive to user-item bipartite graph perturbations.
% In fact, the latest research \cite{SimGCL, XSimGCL, BUIR} empirically inspects that contrastive loss is the primary contributor to boosted performance in CF rather than heuristic-based graph augmentation.
% However, an in-depth understanding of the contrastive loss functions, such as InfoNCE, in the Top-K recommendation, which can theoretically ravel the generalization ability of CL-based recommender, is still limited.
\item \textbf{Limited theoretical understanding for generalization ability in CL-based CF methods.} 
While data augmentation, as a key factor for generalization ability, is pivotal in computer vision \cite{epsilon-delta, ConnectNotCollapse}, the CL-based CF model exhibits insensitivity to perturbations in the user-item bipartite graph \cite{BUIR}. 
Recent studies \cite{SimGCL, XSimGCL} empirically reveal that contrastive loss plays a more crucial role in boosting performance in CF than heuristic-based graph augmentation. 
Yet, a comprehensive theoretical understanding of contrastive loss functions, like InfoNCE, in the realm of Top-K recommendation, which could unravel the generalization ability of CL-based recommenders, remains elusive.
\end{itemize}

\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.325\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/intro1.pdf}
         \caption{$\forall j, s(u,j)-s(u,i)\leq 0$}
         \label{fig:original_condition}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.325\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/intro2.pdf}
         \caption{$s(u,j_1)-s(u,i)\leq -\delta_{j_1}$}
         \label{fig:true_neg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.325\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/intro3.pdf}
         \caption{$s(u,j_2)-s(u,i)\leq -\delta_{j_2}$}
         \label{fig:false_neg}
     \end{subfigure}
        \caption{Comparative geometric interpretation of ranking criteria based on similarity measure $s(\cdot,\cdot)$ for InfoNCE (\ref{fig:original_condition}) and our proposed AdvInfoNCE (\ref{fig:true_neg}-\ref{fig:false_neg}).
        The figures depict the user $u$ as a red dot, with items $i$ (positive), $j_1$ (true negative), and $j_2$ (false negative) depicted as points with varying shades of blue. 
        The color gradient reflects the underlying similarity between user $u$ and the items, while the shaded region delineates the feasible zone for corresponding negative items.}
        \label{fig:ranking_criteria}
        \vspace{-10pt}
\end{figure*}


To better understand and reshape the contrastive loss specially tailored for Top-K recommendation, we aim to automatically and adversarially assign hardness to each negative user-item pair, which de facto concurrently enlarges the similarity discrepancy for hard negatives and loosens the ranking constraint for false negatives.
To be specific, the fundamental idea revolves around discerning a fine-grained degree of hardness for negative interactions, thereby yielding more profound insight into the underlying ranking for Top-K recommendation, as depicted in Figure \ref{fig:ranking_criteria}.
Notably, for a given user $u$, $\delta_j$ refers to the hardness of item $j$.
When $\delta_j > 0$ (as seen in Figure \ref{fig:true_neg}), item $j$ is identified as a hard negative, resulting in a significant contraction of the feasible representation space.
Conversely, when $\delta_j < 0$ (as seen in Figure \ref{fig:false_neg}), the ranking criterion is relaxed compared to the constraint of InfoNCE, allowing the recommender to mitigate the impact of false negative noise. 
Nevertheless, effectively distinguishing between the hard and false negatives and learning a proper and progressively decreasing ranking of interactions continue to present significant challenges \cite{HDCCF}. 

Towards this end, we incorporate a fine-grained degree of hardness for negative interactions and devise a slightly altered version of InfoNCE loss through adversarial training.
This modified contrastive loss coined \textbf{AdvInfoNCE}, is explicitly designed for robust Top-K recommendation. 
Specifically, we frame hardness learning as an adversarial optimization problem by designing a hardness mapping from users/items to negative interaction hardness and iterating between hardness evaluation and CF recommender refinement.

Benefiting from this adversarial framework, our AdvInfoNCE endows two appealing properties.
On the one hand, it serves as a specialized contrastive loss for Top-K collaborative filtering that acknowledges the risk of false negatives while utilizing hard negative mining. 
Additionally, we theoretically demonstrate through adaptive gradients that AdvInfoNCE subtly employs informative negative sampling (\cf \za{Theorem}).
On the other hand, we bridge the adversarial hardness learned by AdvInfoNCE with the ambiguity set in distributionally robust optimization (DRO), thereby naturally demonstrating its generalization ability and assuring its robust performance against the noise of false negatives (\cf \za{Theorem}).
This furnishes a potential theoretical rationalization for the exceptional robustness observed in contrastive learning.
Extensive experiments on out-of-distribution benchmark datasets in Top-K recommendation tasks further highlight the capability of AdvInfoNCE in addressing the issue of biased observations.
We advocate for AdvInfoNCE to be considered a significant reference loss for future contrastive learning research in CF and recommend its adoption as a standard loss in recommender systems.

==> backup/3_method.tex <==
\section{Methodology of AdvInfoNCE}
On the foundation of InfoNCE loss, we first devise AdvInfoNCE, a robust contrastive loss tailor-made for Top-$K$ recommendation scenarios.
Then we present its desirable properties that underscore the efficacy of negative sampling and generalization ability across distribution shifts.

\subsection{Fine-grained Ranking Criterion}
\wx{Instead of the coarse criterion in Equation \eqref{eq:InfoNCE_ranking}, we propose a fine-grained ranking criterion in Top-$K$ recommendation to consider the user preference on different items as compared with the positive items.
It allows us for differentiating between false negatives and hard negatives, and quantifying the relative hardness of each negative item.
Here the hardness of a negative item is defined as its similarity to the positive item, reflecting the relative preference of the user.}

% To learn a fine-grained ranking criterion in Top-$K$ recommendation, rather than relying on the coarse relative ranking criterion presented in Eq \eqref{eq:InfoNCE_ranking}, we need to incorporate the user's varying degrees of preference for different items into the loss function. 
% In other words, we need to differentiate between false negatives and hard negatives, and successfully quantify the relative hardness for each negative instance. 
% Here, the hardness of a negative is defined as its minimal similarity distance towards the positive anchor.

For simplicity, we consider a single observed user-item pair $(u,i) \in \Set{O}^+$ from now on.
Let us assume that for $(u,i)$ pair, we have access to the oracle hardness $\delta_j$ of each negative item $j \in \Set{N}_{u}$.
We can then directly assign distinct hardness values to different negatives and reframe a hardness-aware fine-grained ranking criterion in the semantic similarity space as follows:
\begin{gather} \label{eq:ranking_AdvInfoNCE}
    \forall j \in \Set{N}_u, \quad s(u,j)-s(u,i) + \delta_{j} < 0
\end{gather}
where the hardness $\delta_j \in \Space{R}$. 
If the hardness $\delta_j > 0$ (depicted in Figure \ref{fig:true_neg}), item $j$ is identified as a hard negative, whereas the $\delta_j < 0$ denotes that item $j$ is false negative (depicted in Figure \ref{fig:false_neg}).
The hardness degree offers insight into the user's reversed preference degree, reflecting the personalized ranking. 
This fine-grained ranking criterion provides a level of flexibility surpassing that of InfoNCE's ranking criterion (defined in Eq \eqref{eq:InfoNCE_ranking}).
When an item $j$ is a false negative, the feasible zone expands, indicative of a more relaxed constraint. 
Conversely, when the item $j$ is a hard negative, the feasible zone contracts, corresponding to a stringent constraint that prompts the recommender to focus on this negative item.
In essence, the hardness degree $\delta_j$ encapsulates a fine-grained ranking criterion for user $u$, thereby facilitating a more precise recommendation.

\subsection{Derivation of AdvInfoNCE}
The fine-grained ranking criterion for a single positive interaction $(u,i)$, as defined in Eq
\eqref{eq:ranking_AdvInfoNCE}, can be seamlessly transformed into the main part of our AdvInfoNCE:
\begin{align}
    \underbrace{\max\{0,\{s(u,j)-s(u,i) + \delta_{j}\}_{j\in\Set{N}_u}\}}_{\text{Fine-grained ranking criteria}} \approx \underbrace{- \log \{\frac{\exp(s(u,i))}{\exp(s(u,i))+\sum_{j=1}^{|\Set{N}_u|}\exp(\delta_{j})\exp(s(u,j)) }\}}_{\text{AdvInfoNCE}}  \label{eq:AdvInfoNCE}
\end{align}
In cases where $\forall j, \delta_j=0$, the AdvInfoNCE reverts to InfoNCE loss, as expected.
We outline the main steps of derivation in a brief manner.
For a complete derivation, kindly refer to Appendix \ref{sec:app_derivation_AdvInfoNCE}.

\begin{derivation}
Based on the LogSumExp operation, \ie $\max(x_1,...,x_n) \approx \log(\sum_i \exp(x_i))$, the fine-grained ranking criterion could be approximated in a different form as  $\log (\exp(0)+\sum_{j=1}^{|\Set{N}_u|}\exp(s(u,j)-s(u,i) + \delta_{j}))$. 
Consequently, the right-hand side of Eq \eqref{eq:AdvInfoNCE} can be derived by factoring out the negative sign of the logarithm and reorganizing the term.
\end{derivation}
We would like to highlight the straightforward nature of this derivation, achieved without the need for assumptions, and only utilizing the widely-used LogSumExp operator. 

However, the oracle hardness $\delta_j$ is not accessible or measurable in real-world scenarios.
The challenge, hence, comes to how to automatically learn the appropriate hardness for each negative instance.  
Aiming to enhance robustness in CF methods, we draw inspiration from the adversarial training \cite{Adversarial}.
We integrate a min-max formulation, which allows us to train our model adversarially, alternating between the evaluation of hardness and the refinement of the CF recommender.
Formally, taking into account all observed interactions, we cast the overall framework of the AdvInfoNCE learning strategy  as the following optimization problem:
\begin{align}
    \min_{\theta} \Lapl_{\text{AdvInfoNCE}} = \min_\theta \max_{\Delta\in \Space{C}(\eta)} -\sum_{(u,i)\in\Set{O}^{+}} \log\frac{\exp{(s(u,i))}}{\exp{(s(u,i))}+\sum_{j=1}^{|\Set{N}_u|}\exp(\delta_{j}^{(u,i)})\exp(s(u,j))} 
\end{align}
Here, with a slight abuse of notation, let $\delta_j^{(u,i)}$ denote the relative hardness of negative item $j$ in contrast with interaction $(u, i)$, and $\Delta$ represent the collective set of all $\delta_j^{(u, i)}$.
% The value of $\delta_j$ is bounded by $\Space{C}(\eta)$, where the number of adversarial training epochs is used as the hyperparameter to prevent extreme values and control the deviation.
The definition and enlightening explanation of $\Space{C}(\eta)$ will be presented in section \ref{sec:properties}. 
% \slh{For implementation, we insert a certain number of adversarial training epochs during the training process to learn $\delta_j^{(u, i)}$}. 


\subsection{In-depth Analysis of AdvInfoNCE} \label{sec:properties}
In spite of the adversarial training framework of AdvInfoNCE, the theoretical understanding in terms of its inherent generalization ability remains untouched. 
In this section, we study the robustness of AdvInfoNCE through the lens of distributionally robust optimization (DRO) \cite{DRO_KL} over efficient negative sampling.
From this perspective, AdvInfoNCE focuses on the worst-case distribution over high-quality hard negative sampling.

\begin{restatable}{thm}{DROtheorem} \label{theorem}
We define $\delta_j^{(u,i)} \doteq \log(|\Set{N}_u|\cdot p(j|(u,i)))$, where $p(j|(u,i))$ denotes the probability of sampling negative item $j$ for observed interaction $(u,i)$. 
Then, optimizing AdvInfoNCE loss is \textbf{equivalent} to solving Kullback-Leibler (KL) divergence-constrained distributionally robust optimization (DRO) problems over negative sampling: 
\begin{align}
    \min_\theta\Lapl_{\text{AdvInfoNCE}} \, \Longleftrightarrow  \min_\theta\sup_{p(j|(u,i))\in \Space{P}} \mathbb{E}_P [\exp(s(u,j)-s(u,i)): \Set{D}_{KL}(P||P_0) \leq \eta]
\end{align}
where $P_0$ stands for the distribution of uniformly drawn negative samples, \ie $p_0(j|(u,i)) = \frac{1}{|\Set{N}_u|}$;
$P$ denotes the distribution of negative sampling $p(j|(u,i))$. 
\end{restatable}
For brevity, we present a proof sketch summarizing the key idea here and delegate the full proof to Appendix \ref{sec:app_dro_theorem}.

\begin{proof}
We define $\delta_j^{(u,i)} \doteq \log(|\Set{N}_u|\cdot p(j|(u,i)))$, then $\frac{1}{|\Set{N}_u|}\sum_{j=1}^{|\Set{N}_u|} \delta_l^{(u,i)} = \Set{D}_{KL}(P||P_0)$.
Therefore, by rearranging the terms, optimizing AdvInfoNCE can be restated as a standard DRO problem:
\begin{align}
    \min_\theta\Lapl_{\text{AdvInfoNCE}} & =\min_\theta \max_{\Delta \in \Set{C}(\eta)} \sum_{(u,i)\in\Set{O}^{+}} \log (1+|\Set{N}_u| \sum_{j=1}^{|\Set{N}_u|} p(j|(u,i))\exp(s(u,j)-s(u,i))) \nonumber \\ 
    & \Longleftrightarrow \min_\theta\sup_{p(j|(u,i))\in \Space{P}} \mathbb{E}_P [\exp(s(u,j)-s(u,i))], \, \textrm{s.t.} ~ \Set{D}_{KL}(P||P_0) \leq \eta \nonumber
\end{align}
\end{proof}

We now turn our attention to the role of $\Set{C}(\eta)$ and its relationship with the ambiguity set $\Space{P}$ in DRO. 
The ambiguity set $\Space{P}$ is formulated by requiring the distribution of negative sampling to fall within a certain $\eta$ distance from the uniform distribution, as defined below: 
\begin{align}
    \Space{P} = \{p(j|(u,i))\in (\frac{1}{|\Set{N}_u|}-\epsilon, \frac{1}{|\Set{N}_u|}+\epsilon): \Set{D}_{KL}(P||P_0) \leq \eta = -log(1-\frac{\epsilon^2}{|\Set{N}_u|})\}
\end{align}
where $\epsilon$ serves as the hyperparameter to regulate the deviation of the negative sampling distribution from the uniform distribution. 
In terms of implementation, $\epsilon$ is controlled by the number of adversarial training epochs.
Clearly, $\Set{C}(\eta)$ is an equal counterpart to the ambiguity set $\Space{P}$.

\textbf{Discussion.}
Grounded by theoretical proof, we understand the generalization ability of our AdvInfoNCE through the lens of DRO over informative negative sampling. 
In essence, by learning the hardness in an adversarial manner, AdvInfoNCE effectively enhances the robustness of the CF recommender.
Moreover, apart from the robustness of AdvInfoNCE (see Section \ref{sec:properties}), we also identify its hard negative mining mechanism through gradients analysis (see Appendix \ref{sec:app_negative_ming}) and its alignment with Top-$K$ ranking evaluation metrics (see Appendix \ref{sec:app_topK}).
Specifically, the gradients concerning negative samples are proportional to the hardness term $\exp(\delta_j)$, indicating that AdvInfoNCE is a hardness-aware loss.
To some extent, our AdvInfoNCE is equivalent to the widely-adopted Discounted Cumulative Grain (DCG) ranking metric.

\textbf{Limitation.}
AdvInfoNCE employs end-to-end negative sampling in an adversarial manner, compelling the recommender to ensure robustness from the worst-case scenario. 
Despite its empirical success and desirable properties, AdvInfoNCE is not immune to the limitations of adversarial training, which is well-known for its potential training instability and sensitivity to parameters.


==> chapters/5_related_work.tex <==
\section{Related Work}

\textbf{Negative Sampling}

\textbf{Theoretical Understanding of Contrastive Loss in Recommender System}
